Reasoning with Finite Sets and Cardinality Constraints in SMT

We consider the problem of deciding the satisfiability of quantifier-free formulas in the theory of finite sets with cardinality constraints. Sets are a common high-level data structure used in programming; thus, such a theory is useful for modeling program constructs directly. More importantly, sets are a basic construct of mathematics and thus natural to use when formalizing the properties of computational systems. We develop a calculus describing a modular combination of a procedure for reasoning about membership constraints with a procedure for reasoning about cardinality constraints. Cardinality reasoning involves tracking how different sets overlap. For efficiency, we avoid considering Venn regions directly, as done in previous work. Instead, we develop a novel technique wherein potentially overlapping regions are considered incrementally as needed, using a graph to track the interaction among the different regions. The calculus has been designed to facilitate its implementation within SMT solvers based on the DPLL($T$) architecture. Our experimental results demonstrate that the new techniques are competitive with previous techniques and can scale much better on certain classes of problems.

==> Makefile <==
FILE=pap

compile:
	pdflatex -interaction=nonstopmode $(FILE)
	bibtex $(FILE)
	pdflatex $(FILE)
	pdflatex $(FILE)

auto:
	trap exit INT; while true; do \
	  pdflatex -interaction=nonstopmode $(FILE); \
	  if [ -n "$(shell which inotifywait)" ]; then \
	    inotifywait *.tex; \
	  elif [ -n "$(shell which fswatch)" ]; then \
	    fswatch -1 *.tex; \
	  else \
	    echo "Need inotifywait or fswatch installed"; break; \
	  fi; \
	done

spell:
	hunspell -l -t -i utf-8 -p wordlist.txt *.tex

clean:
	-rm -f $(FILE).aux
	-rm -f $(FILE).bbl
	-rm -f $(FILE).blg
	-rm -f $(FILE).log
	-rm -f $(FILE).out

#clean:
#	rm -f FILEwait*



==> prop-graph.tex <==
\begin{proof}[Proof (Proposition \ref{prop:graph}, property \ref{prop:graph:propequal})]
Let $\aset \opequal \bset \in \setconst$, with $\aset \in \vertices$ or $\bset \in \vertices$.
From rule \ruleIntroEqRight and rule \ruleIntroEqLeft it follows that both $\aset \in \vertices$ and $\bset \in \vertices$.
%
For each of the Rules \ruleMergeEqI, \ruleMergeEqII, and \ruleMergeEqIII; we show that
after the application of the rule, $\nonemptyleaves{s}$ and $\nonemptyleaves{t}$ are equal.
%\begin{itemize}
%\item

Consider rule \ruleMergeEqI.
Let $L_\aset$ and $L_\bset$ denote $\nonemptyleaves{\aset}$ and $\nonemptyleaves{\bset}$ respectively
before application of the rule. Let $L'_\aset$ and $L'_\bset$ denote
$\nonemptyleaves{\aset}$ and $\nonemptyleaves{\bset}$ after application of the rule.
%
For the rule to be applicable $L_\aset \subsetneq L_\bset$.
The rule adds constraints to $\setconst$ so that $L'_\bset = L_\bset \setminus (L_{\bset} \setminus L_\aset)$.
Equivalently, $L'_\bset = L_\bset \cap L_\aset = L_\aset$. Since $L'_\aset = L_\aset$,
we get $L'_\aset = L_\aset = L'_\bset$.

%\item
The case for rule \ruleMergeEqII~is analogous to rule \ruleMergeEqI.

%\item
Consider rule \ruleMergeEqIII.
Let $L_\aset$ and $L_\bset$ denote $\nonemptyleaves{\aset}$ and $\nonemptyleaves{\bset}$ respectively
before application of the rule. Let $L'_\aset$ and $L'_\bset$ denote
$\nonemptyleaves{\aset}$ and $\nonemptyleaves{\bset}$ after application of the rule.
%
Let $n \in L'_\aset$. Note that the $\merge$ operation only adds nodes
and vertices. Thus, $n$ is one of the following:
\begin{itemize}
\item $l_1 \opinter l_2$ with $l_1 \in L_\aset$ and $l_2 \in L_\bset$:
  Since $(l_1, l_1 \opinter l_2)$ as well as $(l_2, l_1 \opinter l_2)$ is an edge, it follows that $n \in L'_\bset$.
\item $l_1 \in L_\aset$. Since nodes in $L_\aset \setminus L_\bset$ have an outgoing edge, it must be the case that $l_1 \in L_\aset \cap L_\bset$. It follows that $n \in L'_\bset$.
\end{itemize}
This shows that $L'_\aset \subseteq L'_\bset$. The reasoning for $L'_\bset \subseteq L'_\aset$ is symmetrical.
%\end{itemize}

As $\aset \opequal \bset$, $\aset \in \vertices$, and $\bset \in \vertices$, the premise of at least
once of the rules (\ruleMergeEqI), (\ruleMergeEqII), and (\ruleMergeEqIII) must be satisfied
whenever $\nonemptyleaves{s} \neq \nonemptyleaves{t}$.
As the branch is saturated, $\nonemptyleaves{s} = \nonemptyleaves{t}$ follows.
\end{proof}
%\item
%
\begin{proof}[Proof (Proposition \ref{prop:graph}, properties \ref{prop:graph:propunion}, \ref{prop:graph:propinter}, \ref{prop:graph:propsetminus})]

As $\derivtree$ is obtained from a derivation starting with a state
with an empty graph, it is sufficient to show the properties hold for
the empty graph, and that they are preserved each time the graph is
modified by one of the rules.

The properties hold trivially for the empty graph. The interesting
cases are when edges are added to the graph: i) $\add$ of a union,
intersection, or set minus term, and ii) $\merge$ operation.

Observe that when we introduce $T \opunion U$,  $T \opinter U$, and  $T \opsetminus U$ to the graph:
\begin{itemize}
\item $\leaves{T} = \{T \opsetminus U, T \opinter U\}$,
\item $\leaves{U}= \{T \opinter U, U \opsetminus T\}$,
\item  $\leaves{T \opunion U} = \{ T \opsetminus U,  T \opinter U, U \opsetminus T\}$,
\item  $\leaves{T \opinter U} = \{ T \opinter U \}$,
\item $\leaves{T \opsetminus U} = \{T \opsetminus U\}$, and
\item $\leaves{U \opsetminus T} = \{U \opsetminus T\}$.
\end{itemize}
We conclude that:
\begin{itemize}
\item $\leaves{T \opunion U} = \leaves{T} \cup \leaves{U}$
\item $\leaves{T \opinter U} = \leaves{T} \cap \leaves{U}$
\item $\leaves{T \opsetminus U} = \leaves{T} \setminus \leaves{U}$
\item $\leaves{U \opsetminus T} = \leaves{U} \setminus \leaves{T}$
\end{itemize}
when an introduce rule is applied.
%
Note that the merge operation only adds edges from existing leaf
nodes, ensuring that the property is maintained by any application
of $\merge$.

$\nonemptyleaves{\cdot}$, as defined in (\ref{eq:nonemptyleaves}), can also be defined as:
\begin{equation}
  \nonemptyleaves{n} = \leaves{n} \setminus E
\end{equation}
where $E = \setbuilder{n' \in \vertices}{n' \opequal \opemptyset \in \setconstclosed}$
does not depend on $n$.
The properties in the proposition about $\nonemptyleaves{\cdot}$
follow from the corresponding property of $\leaves{\cdot}$ just established, and
above formulation of $\nonemptyleaves{\cdot}$.
\end{proof}
%% \item Let $\aset \in \vertices$.
%%   For all $\bset, \cset \in \leaves{\aset}$, $\bset \neq \cset$, the two sets are necessarily disjoint:
%%   \[ \models_\settheory  \bset \opinter \cset \opequal \opemptyset\text{.} \]
\begin{proof}[Proof (Proposition \ref{prop:graph}, properties \ref{prop:graph:propdisjoint},\ref{prop:graph:propleaves})]
The properties holds trivially for the empty graph.

Let $\graphconst$ be the graph constraints. Let $\aset \in \vertices$.
%
Let $\aset' \opequal \emptyset$ be a new constraint such that $\aset' \in \nonemptyleaves{\aset}$.
Then, this modifies $\nonemptyleaves{\aset}$, and we need to verify the Property \ref{prop:graph:propleaves} still holds.
%% Property \ref{prop:graph:propdisjoint} is not affected,
%% the interesting case is property \ref{prop:graph:propleaves}.
%% If
%% \[\models_\settheory \inparen{\bigwedge_{\bset \in E} \bset \opequal \opemptyset} \Rightarrow \aformula \quad\text{,}\]
%% then
%% \[\inparen{\aset' \opequal \opemptyset \wedge \bigwedge_{\bset \in E} \bset \opequal \opemptyset} \Rightarrow \aformula \quad\text{.}\]
Note that for any structure in $\settheory$, if $\aset'$ is interpreted as empty set, the interpretation of
$\bigsqcup_{\bset \in \nonemptyleaves{\aset} \setminus \{\aset'\}} \bset$
will be same as $\bigsqcup_{\bset \in \nonemptyleaves{\aset}} \bset$.
Thus, if $\aset' \in \nonemptyleaves{\aset}$ and
\[ \models_\settheory \inparen{\bigwedge_{P \in E} P} \Rightarrow \inparen{\aset \opequal \bigsqcup_{\bset \in \nonemptyleaves{\aset}} \bset} \quad\text{,}\]
then
 \[ \models_\settheory \inparen{\aset' \opequal \opemptyset \wedge \bigwedge_{P \in E} P} \Rightarrow \inparen{\aset \opequal \bigsqcup_{\bset \in \nonemptyleaves{\aset} \setminus \{\aset'\}} \bset} \quad\text{.}\]
It follows if $\aset' \opequal \emptyset$ is added to $\setconstclosed$ by a rule, the property \ref{prop:graph:propleaves} continue to hold.
Also note that a equality is not removed by any rule (if there was such a rule, we'd need to check the property continues to hold when the left side of the implication is weakened).

The only other rules which affect the properties are those which modify the graph directly,
i.e. the $\add$ and $\merge$ operations.

We show that if $\graphconst$ satisfies the properties, then so does $\add(\graphconst, \aset)$:
\begin{itemize}
\item $\aset$ is $\opemptyset$, $\asetv$ or $\opsingleton{x}$: trivially, as no edges are added.
\item $\aset$ is $\bsetv \opinter \csetv$:
  Note that because of the assumptions on the normal form, either $\bsetv \opinter \csetv$ already in the graph and $\add$
  operation does not modify the graph, or it will add the nodes $\bsetv$, $\csetv$, $\bsetv \opsetminus \csetv$, $\bsetv \opinter \csetv$,
  and $\csetv \opsetminus \bsetv$ to the graph, and edges between them.
%\ksays{The assumption does not give this unfortunately. Normal form still needs
%to be adjusted. Merge can add edges.}
 It is easy to see that the property \ref{prop:graph:propdisjoint} follows from:
  \begin{align*}
    &\models_\settheory \inparen{\inparen{\bsetv \opsetminus \csetv} \opinter \inparen{\bsetv \opinter \csetv}} \opequal \opemptyset \\
    &\models_\settheory \inparen{\inparen{\csetv \opsetminus \bsetv} \opinter \inparen{\bsetv \opinter \csetv}} \opequal \opemptyset
  \end{align*}
  Property \ref{prop:graph:propleaves} follows from:
  \begin{align*}
    &\models_\settheory \bsetv \opequal \inparen{\inparen{\bsetv \opsetminus \csetv} \opunion \inparen{\bsetv \opinter \csetv}} \\
    &\models_\settheory \csetv \opequal \inparen{\inparen{\csetv \opsetminus \bsetv} \opunion \inparen{\bsetv \opinter \csetv}} \\
    &\models_\settheory \inparen{\bsetv \opinter \csetv} \opequal \inparen{\bsetv \opinter \csetv} \\
    &\models_\settheory \inparen{\csetv \opsetminus \bsetv} \opequal \inparen{\csetv \opsetminus \bsetv} \\
    &\models_\settheory \inparen{\bsetv \opsetminus \csetv} \opequal \inparen{\bsetv \opsetminus \csetv}
  \end{align*}
  and reasoning as earlier that any constraint of the form $\aset' \opequal \opemptyset$ does not affect the property.
\item $\aset$ is $\bsetv \opsetminus \csetv$ or $\csetv \opsetminus \bsetv$: reasoning same as for $\bsetv \opinter \csetv$.
\item $\aset$ is $\bsetv \opunion \csetv$. If not already present, $\bsetv$, $\csetv$, $\bsetv \opsetminus \csetv$, $\bsetv \opinter \csetv$ are added to the graph as for $\bsetv \opinter \csetv$. In addition, $\add$ for union also adds $\bsetv \opunion \csetv$, and three edges. The properties follows from the following tautologies in $\settheory$ in addition to those listed in analysis for $\bsetv \opinter \csetv$:
  \begin{align*}
    &\models_\settheory \inparen{\inparen{\bsetv \opsetminus \csetv} \opinter \inparen{\inparen{\csetv \opsetminus \bsetv}}} \opequal \opemptyset \\
    &\models_\settheory \inparen{\bsetv \opunion \csetv} \opequal \inparen{\inparen{\bsetv \opsetminus \csetv} \opunion \inparen{\bsetv \opinter \csetv} \opunion \inparen{\csetv \opsetminus \bsetv}}
  \end{align*}
\end{itemize}

Finally, we show that if $\graphconst$ satisfies the properties,
then so does $\merge(\graphconst, \aset, \bset)$ if
$\aset \in \vertices$,
$\bset \in \vertices$,
$\nonemptyleaves{\aset} \nsubseteq \nonemptyleaves{\bset}$ and
$\nonemptyleaves{\bset} \nsubseteq \nonemptyleaves{\aset}$.

Let $L_\aset$ denote $\nonemptyleaves{\aset}$ in $\graphconst$,
and $L'_\aset$ denote $\nonemptyleaves{\aset}$ in $\merge(\graphconst, \aset', \bset')$
(likewise for $\bset$, $\cset$ etc.).

In order to show property \ref{prop:graph:propdisjoint} holds,
let $\aset' \in \vertices$, $\bset' \in L'_{\aset'}$ and $\cset' \in L'_{\aset'}$.
We need to show:
$\models_\settheory \bset' \opinter \cset' \opequal \opemptyset$.
\begin{itemize}
\item Let $\bset' \in L_{\aset'}$ and $\cset' \in L_{\aset'}$, i.e. both are
  also leaf nodes in $\graphconst$. Then, the property for $\merge(\graphconst, \aset, \bset)$
  follows from that of $\graphconst$.
\item Let $\bset'$ be one of the newly introduced leaf nodes and $\cset' \in L_{\aset'}$ a leaf node in $\graphconst$.
  Without loss of generality, let $\bset'$ be $t_1 \opinter t_2$
  with $t_1 \in L_\aset \setminus L_\bset$ and $t_2 \in L_\bset \setminus L_\aset$.
  For $\bset'$ to be in $L'_{\aset'}$, given the way the edges are added, either
  $t_1 \in L_{\aset'}$ or $t_2 \in L_{\aset'}$. Thus, we know that either
  $\models_\settheory t_1 \opinter \cset' \opequal \opemptyset$
  or
  $\models_\settheory t_2 \opinter \cset' \opequal \opemptyset$.
  In either case, it follows that
  $\models_\settheory \inparen{t_1 \opinter t_2} \opinter \cset' \opequal \opemptyset$, i.e.
  $\models_\settheory \bset' \opinter \cset' \opequal \opemptyset$.
\item The analysis for the case where both are newly introduced leaf nodes is similar.
\end{itemize}

To show property \ref{prop:graph:propleaves} holds,
the main observation is that each node no longer a leaf node, say $\aset' \in L_{\aset} \setminus L'_{\aset}$,
is union of a new set of leaf nodes in $L'_{\aset}$ (assuming the equalities).
\begin{align*}
  \aset'
  & \opequal \aset' \opinter \aset
  & \text{($\aset' \in L_\aset$, $\aset \opequal \bigsqcup_{\aset'' \in L_\aset} \aset''$)}
  \\
  & \opequal \aset' \opinter \bset
  & \text{($\aset \opequal \bset \in E$)}
  \\
  & \opequal \aset' \opinter \inparen{\bigsqcup_{\bset' \in L_\bset} \bset'}
  & \text{($\bset \opequal \bigsqcup_{\bset' \in L_\bset} \bset'$)}
  \\
  & \opequal \bigsqcup_{\bset' \in L_\bset} \aset' \opinter \bset'
  & \text{(distribute)}
  \\
  \intertext{But by property \ref{prop:graph:propdisjoint}, $\aset' \opinter \bset' \opequal \opemptyset$ for $\aset', \bset' \in L_\aset$. Thus,}
  \aset'
  & \opequal \bigsqcup_{\bset' \in L_\bset \setminus L_\aset} \aset' \opinter \bset'
\end{align*}
Note that $\setbuilder{\aset' \opinter \bset'}{\bset'\in L_\bset \setminus L_\aset}$ are precisely the nodes in
$L'_\aset$ to which edges are added from $\aset'$. The proof for a node in $L_{\bset}$ but not in $L'_{\bset}$ is similar.

Since all the new leaf nodes are of the form $\aset' \opinter \bset'$ with $\aset'\in L_\aset \setminus L_\bset$ and
$\bset'\in L_\bset \setminus L_\aset$, it follows that property \ref{prop:graph:propleaves} holds for $\merge(\graphconst, \aset, \bset)$ if
it holds for $\graphconst$ assuming $\aset \opequal \bset \in E$.
%
%% \item Let $\aset \in \vertices$. Let $E = \setbuilder{\bset \in \vertices}{\bset \opequal \opemptyset \in \setconstclosed}$.
%%   Then\footnote{Technically, $\bigsqcup_{\ldots}$ is ambiguous. But, in any interpretation in $\settheory$, the interpretation of $\opunion$ is associative, so the bracketing does not matter in our context.}
%%   \begin{equation}
%%   \models_\settheory \inparen{\bigwedge_{\bset \in E} \bset \opequal \opemptyset}
%%   \Rightarrow
%%   \inparen{\aset \opequal \bigsqcup_{\bset \in \nonemptyleaves{\aset}} \bset}
%%   \label{eq:nodeLeavesReln}
%%   \end{equation}
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "pap.tex"
%%% End:

